Discrete spectrum of the magnetic Laplacian on perturbed half-planes

The existence of bound states for the magnetic Laplacian in unbounded domains can be quite challenging in the case of a homogeneous magnetic field. We provide an affirmative answer for almost flat corners and slightly curved half-planes when the total curvature of the boundary is positive.

==> biblio.tex <==


@article {BMR14,
	AUTHOR = {Bruneau, Vincent and Miranda, Pablo and Raikov, Georgi},
	TITLE = {Dirichlet and {N}eumann eigenvalues for half-plane magnetic
		{H}amiltonians},
	JOURNAL = {Rev. Math. Phys.},
	FJOURNAL = {Reviews in Mathematical Physics. A Journal for Both Review and
		Original Research Papers in the Field of Mathematical Physics},
	VOLUME = {26},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {1450003, 23},
	ISSN = {0129-055X},
	MRCLASS = {47F05 (35J10 35P20 35Q40 81Q10)},
	MRNUMBER = {3190206},
	DOI = {10.1142/S0129055X14500032},
	URL = {https://doi.org/10.1142/S0129055X14500032},
}

@article {BN,
	AUTHOR = {Bonnaillie, Virginie},
	TITLE = {On the fundamental state energy for a {S}chr\"{o}dinger operator
		with magnetic field in domains with corners},
	JOURNAL = {Asymptot. Anal.},
	FJOURNAL = {Asymptotic Analysis},
	VOLUME = {41},
	YEAR = {2005},
	NUMBER = {3-4},
	PAGES = {215--258},
	ISSN = {0921-7134},
	MRCLASS = {35Q55 (78A02 81Q05)},
	MRNUMBER = {2127997},
	MRREVIEWER = {Tiziana Giorgi},
}

@article {CG,
	AUTHOR = {Correggi, Michele and Giacomelli, Emanuela L.},
	TITLE = {Almost flat angles in surface superconductivity},
	JOURNAL = {Nonlinearity},
	FJOURNAL = {Nonlinearity},
	VOLUME = {34},
	YEAR = {2021},
	NUMBER = {11},
	PAGES = {7633--7661},
	ISSN = {0951-7715},
	MRCLASS = {35Q56},
	MRNUMBER = {4321415},
	DOI = {10.1088/1361-6544/ac24e0},
	URL = {https://doi.org/10.1088/1361-6544/ac24e0},
}

@article {Eetal,
	AUTHOR = {Exner, Pavel and Lotoreichik, Vladimir and P\'{e}rez-Obiol, Axel},
	TITLE = {On the bound states of magnetic {L}aplacians on wedges},
	JOURNAL = {Rep. Math. Phys.},
	FJOURNAL = {Reports on Mathematical Physics},
	VOLUME = {82},
	YEAR = {2018},
	NUMBER = {2},
	PAGES = {161--185},
	ISSN = {0034-4877},
	MRCLASS = {35P05 (35J05 35J10 47F05)},
	MRNUMBER = {3906610},
	MRREVIEWER = {Rupert L. Frank},
	DOI = {10.1016/S0034-4877(18)30084-3},
	URL = {https://doi.org/10.1016/S0034-4877(18)30084-3},
}

@article {FH06,
	AUTHOR = {Fournais, Soeren and Helffer, Bernard},
	TITLE = {Accurate eigenvalue asymptotics for the magnetic {N}eumann
		{L}aplacian},
	JOURNAL = {Ann. Inst. Fourier (Grenoble)},
	FJOURNAL = {Universit\'{e} de Grenoble. Annales de l'Institut Fourier},
	VOLUME = {56},
	YEAR = {2006},
	NUMBER = {1},
	PAGES = {1--67},
	ISSN = {0373-0956},
	MRCLASS = {35Q40 (35P15 35P20 47F05 47N50 81Q20 82D55)},
	MRNUMBER = {2228679},
	MRREVIEWER = {Michael Melgaard},
	URL = {http://aif.cedram.org/item?id=AIF_2006__56_1_1_0},
}

@article {HK17,
	AUTHOR = {Helffer, Bernard and Kachmar, Ayman},
	TITLE = {Eigenvalues for the {R}obin {L}aplacian in domains with
		variable curvature},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {369},
	YEAR = {2017},
	NUMBER = {5},
	PAGES = {3253--3287},
	ISSN = {0002-9947},
	MRCLASS = {35P15 (35J05 47F05)},
	MRNUMBER = {3605971},
	MRREVIEWER = {J. B. Kennedy},
	DOI = {10.1090/tran/6743},
	URL = {https://doi.org/10.1090/tran/6743},
}



@article {BHR22,
	AUTHOR = {Bonnaillie-No\"{e}l, Virginie and H\'{e}rau, Fr\'{e}d\'{e}ric and Raymond,
		Nicolas},
	TITLE = {Purely magnetic tunneling effect in two dimensions},
	JOURNAL = {Invent. Math.},
	FJOURNAL = {Inventiones Mathematicae},
	VOLUME = {227},
	YEAR = {2022},
	NUMBER = {2},
	PAGES = {745--793},
	ISSN = {0020-9910},
	MRCLASS = {Prelim},
	MRNUMBER = {4372223},
	DOI = {10.1007/s00222-021-01073-x},
	URL = {https://doi.org/10.1007/s00222-021-01073-x},
}

@article {R13,
	AUTHOR = {Raymond, Nicolas},
	TITLE = {From the {L}aplacian with variable magnetic field to the
	electric {L}aplacian in the semiclassical limit},
	JOURNAL = {Anal. PDE},
	FJOURNAL = {Analysis \& PDE},
	VOLUME = {6},
	YEAR = {2013},
	NUMBER = {6},
	PAGES = {1289--1326},
	ISSN = {2157-5045},
	MRCLASS = {35J10 (35B25 35C20 35P15)},
	MRNUMBER = {3148056},
	MRREVIEWER = {Michael A. Perelmuter},
	DOI = {10.2140/apde.2013.6.1289},
	URL = {https://doi.org/10.2140/apde.2013.6.1289},
}



@article {Simon,
	AUTHOR = {Simon, Barry},
	TITLE = {The bound state of weakly coupled {S}chr\"{o}dinger operators in
	one and two dimensions},
	JOURNAL = {Ann. Physics},
	FJOURNAL = {Annals of Physics},
	VOLUME = {97},
	YEAR = {1976},
	NUMBER = {2},
	PAGES = {279--288},
	ISSN = {0003-4916},
	MRCLASS = {35J10},
	MRNUMBER = {404846},
	MRREVIEWER = {M. S. P. Eastham},
	DOI = {10.1016/0003-4916(76)90038-5},
	URL = {https://doi.org/10.1016/0003-4916(76)90038-5},
}



@book {FH10,
	AUTHOR = {Fournais, S{\o}ren and Helffer, Bernard},
	TITLE = {Spectral methods in surface superconductivity},
	SERIES = {Progress in Nonlinear Differential Equations and their
	Applications},
	VOLUME = {77},
	PUBLISHER = {Birkh\"{a}user Boston, Inc., Boston, MA},
	YEAR = {2010},
	PAGES = {xx+324},
	ISBN = {978-0-8176-4796-4},
	MRCLASS = {35-02 (35P15 35Q56 47F05 47N50 49N60 82D55)},
	MRNUMBER = {2662319},
	MRREVIEWER = {Yuri A. Kordyukov},
}

@book {Raymond,
	AUTHOR = {Raymond, Nicolas},
	TITLE = {Bound states of the magnetic {S}chr\"{o}dinger operator},
	SERIES = {EMS Tracts in Mathematics},
	VOLUME = {27},
	PUBLISHER = {European Mathematical Society (EMS), Z\"{u}rich},
	YEAR = {2017},
	PAGES = {xiv+380},
	ISBN = {978-3-03719-169-9},
	MRCLASS = {35-02 (35P15 35P20 35Q60 81-02 81Q12)},
	MRNUMBER = {3616340},
	MRREVIEWER = {Joseph L. Shomberg},
	DOI = {10.4171/169},
	URL = {https://doi.org/10.4171/169},
}


